The B-meson mass splitting from non-perturbative quenched lattice QCD

We perform the non-perturbative (quenched) renormalization of the chromo-magnetic operator in Heavy Quark Effective Theory and its three-loop matching to QCD. At order 1/m of the expansion, the operator is responsible for the mass splitting between the pseudoscalar and vector B-mesons. These new computed factors are affected by an uncertainty negligible in comparison to the known bare matrix element of the operator between B-states. Furthermore, they push the quenched determination of the spin splitting for the Bs-meson much closer to its experimental value than the previous perturbatively renormalized computations. The renormalization factor for three commonly used heavy quark actions and the Wilson gauge action and useful parametrizations of the matching coefficient are provided.

==> table_zlref.tex <==
\begin{table}
\small{
\begin{center}
\begin{tabular}{cc|cc|cc|cc}
\hline 
$\beta$ & $L / a$   & action  & $\zmagsf$ & action  & $\zmagsf$ 
& action  & $\zmagsf$\\
\hline
6.0219& 8   &  EH &2.585(19)  & HYP1 &2.553(20) & HYP2 &2.593(21)  \\ 
6.1628& 10  &  EH &2.602(24)  & HYP1 &2.575(24) & HYP2 &2.589(26)  \\
6.2885& 12  &  EH &2.602(24)  & HYP1 &2.558(22) & HYP2 &2.589(26)  \\
6.3992& 14  &  EH &2.589(29)  & HYP1 &2.553(24) & HYP2 &2.585(21)  \\
6.4956& 16  &  EH &2.593(35)  & HYP1 &2.533(27) & HYP2 &2.553(22)  \\
\hline
\end{tabular}
\caption{%\footnotesize 
Renormalization factor at the matching scale $\mu=1/2L_{\rm max}$. 
In all cases $\hat{F}_{\mu\nu}$ is the standard (not smeared)
clover operator. The actions are defined as in \cite{Della_Morte:2005yc}. The HYP1 results are new with respect to \cite{Guazzini:2007bu}.}
\label{t:zlref}
\end{center}
}
\end{table}
